Phenomenology of baryon dynamics with directed flow in relativistic heavy-ion collisions

This thesis aims to elucidate the role of initial baryon stopping and its diffusion in heavy-ion collisions (HIC) using hydrodynamic model. In this regard, we have studied the observable-directed flow ($v_1$) of identified hadrons, particularly the $v_1$ of baryons and antibaryons, as well as the splitting observed between them in detail. We propose a new ansatz for the initial baryon distribution. By employing this initial baryon deposition model alongside a tilted energy distribution as inputs to a hybrid framework, we successfully describe the rapidity-odd $v_1$ of identified hadrons, including the elusive baryon-antibaryon splitting of $v_1$ across a wide range of $\sqrt{s_{NN}}$. Our model, incorporating baryon stopping and it's subsequent diffusion within a relativistic hydrodynamic framework and employing a crossover equation of state derived from lattice QCD calculations, establishes a non-critical baryonic baseline. Moreover, we demonstrate that recent STAR measurements of the centrality and system-size dependence of $v_1$ splitting between oppositely charged hadrons-attributed to electromagnetic field effects-are significantly influenced by background contributions from baryon stopping and its diffusion. Furthermore, we show that the rapidity dependence of the splitting of the rapidity-even component of $v_1$ between $p$ and $\bar{p}$ is highly sensitive to the initial baryon deposition scheme. If measured experimentally, this could constraint the rapidity dependence of the initial baryon deposition profile. Moreover, it could offer valuable phenomenological insights into the baryon junction picture and help refine constraints on the baryon diffusion coefficient of the medium. Notably, utilizing this phenomenologically successful baryon deposition model, we present the first estimation of the baryon diffusion coefficient for the strongly interacting QCD matter created in HIC.

==> chapters/acknowledgments.tex <==
\chapter{Acknowledgements}
I would like to express my sincere gratitude to IISER Berhampur for providing financial support through the institute fellowship and access to computational facilities, which were essential for carrying out my research work. I extend my heartfelt thanks to my thesis supervisor, Dr. Sandeep Chatterjee. He has been not only a teacher and collaborator but also a motivator, supporter, senior, guardian, critic, resilience trainer, and endurance coach in the field of research for me. I sincerely appreciate him for introducing me to an engaging and cutting-edge research topic, which served as the cornerstone of my PhD thesis. I am also deeply thankful to my research collaborators, Dr. Md Nasim, Prof. Piotr Bożek, Prof. Jean-Yves Ollitrault, and Dr. Rupam Samanta, from whom I gained profound insights into the fascinating physics of heavy-ion collisions, including aspects beyond the scope of my PhD topic. Their valuable inputs have significantly enriched my understanding of the subject.


I am also grateful to my Research Progress Committee members, Dr. Md. Nasim, Dr. Sayantan Sharma, and Dr. Ujjal Kumar Dey, for evaluating my progress and providing invaluable comments and suggestions. My sincere thanks also go to Prof. Sourendu Gupta, Dr. Subhash Singha, and Dr. Amaresh Jaiswal for their insightful advice and guidance.

I would like to express my gratitude to all the members of the Heavy-Ion Physics group at IISER Berhampur who were present during my PhD tenure. Engaging in discussions with them significantly enhanced my understanding of the subject. I am thankful to the group memebers Dr. Sandeep Chatterjee, Dr. Md. Nasim, Dr. Natasha Sharma, Dr. Vipul Bairathi, Dr. Ashutosh Dash, Dr. Nachiketa Sarkar, Dr. Surashree Majumdar, Mr. Kaiser Shafi, Mr. Prabhupada Dixit, Mr. Aswini Kumar Sahoo, Ms. Aradhana Pandey, Ms. Priya, Mr. Pranjal Barik, Mr. Sourav Bera, Mr. Koustav Maity, Mr. Sanataun Prodhan, Mr. Harish Avuddaiyapan, Mr. Betha LGR Manjunath, Mr. Arkadip Mukherjee, Mr. Abhisek Praharaj, and Mr. Jayanta Naik.


I would like to express my gratitude to Dr. Vipul Bairathi, who introduced me to various computational techniques during the early stages of my research. I am deeply thankful to the trio—Koustav, Sourav, and Santanu—for instilling a competitive mindset in me at a critical point in my PhD journey, an experience I will never forget. I also appreciate Dr. Ashutosh Dash, whose brief yet impactful time at IISER Berhampur greatly influenced me. Our long discussions significantly enhanced my physics insights, and I drew inspiration from his work and from his passion to research. I am also grateful to Mr. Kasinath Dash. My discussions with him greatly contributed to my understanding of general physics.

I am very grateful to my friend and colleague, Mr. Kaiser Shafi, who has been a constant source of support. Whenever I needed to scrutinize my write-ups or slides in detail, I would always turn to him. His valuable suggestions and meticulous corrections, given generously with his time, were incredibly helpful. He has a remarkable attention to detail, and I admire his efforts in testing many of my codes, identifying errors, and pointing out unnecessary complexities. His suggestions greatly improved the quality of my work and helped me reduce errors.

Explaining concepts to my experimentalist friends, Aswini and Prabhupada, also deepened my understanding of the subject. I am grateful for their patience in listening to my ideas and research, often over tea. They frequently pointed out errors or misinterpretations in my understanding of certain phenomena, and their insightful and thought-provoking questions challenged me to think more critically and improve. Their suggestions have always been invaluable.

My two-month research visit to Dr. Subhash Singha at IMP, China, was a pivotal phase of my PhD. The working environment there played a crucial role in providing the final touch to my thesis work. It not only boosted my motivation but also helped me gain a clearer outlook on my future research endeavors. Additionally, I had the opportunity to collaborately work with Dr. Singha and to explore more interesting topics in heavy-ion physics. I am truly grateful to him for this valuable experience.

I am thankful to Prof. Raghunath Sahoo, who initially in my MSc. days motivated me to pursue research in heavy-ion collisions. I also appreciate his PhD student Dr. Arvind Khuntia for his valuable advice and for explaining the field in detail that time. His suggestion was really helpful.

I am grateful to Prof. Rohit Soni and Dr. Somenath Kale for their unwavering support. It is hard to imagine the speed of my research work without their assistance.

I would like to express my gratitude to the teachers from my undergraduate and postgraduate years. It is because of them that I have had the opportunity to learn and explore the beautiful subject of physics. 


I truly believe I was fortunate to have Nimish, Aswini, and Prabhupada as my friends during my PhD journey. I cannot imagine my PhD experience without them. I am deeply grateful to these fun, entertaining, and supportive friends who helped me cope with the pressures of work. My family, hundreds of kilometers away, and Mr. Sandeep, who was always concerned about my health, especially after the severe COVID-19 attack I suffered, were reassured knowing that Mr. Nimish was there for me in any medical emergency. I also cherish the weekends spent with the funniest person I’ve ever known, Mr. Prabhupada. I am constantly amazed by how he manages to stay calm and humorous in every situation. Additionally, the cheerful gatherings at Ganjam Dhaba or Room No. 65 would never have been as lively without the light-hearted presence of Aswini. His ability to not take a joke to heart is remarkable—a trait not everyone can master. His charm is truly hard to match.


My brother, Lipu, has been my most steadfast and unspoken supporter. His expectations from me continue to drive and motivate me. I am at a loss for words when it comes to expressing my gratitude to my father and mother. All I can say is that being worthy of writing an acknowledgment section in a PhD dissertation would not have been possible without their unwavering support and sacrifice. I also wish to thank my close friends, Biswajit Panda, Biswajit Biswal, Prabhudatta, Durga, Anakar, Amit, Rakun, and Budha for their constant support and for reminding me to believe in myself. Additionally, I am thankful to all the inspiring individuals from my village, Juanga, who have always encouraged me to grow and improve.


"Be professional, not emotional.". The line inspired me the most.






==> chapters/certificate.tex <==
\chapter*{CERTIFICATE OF APPROVAL}
Certified that the thesis entitled \textbf{\textit{"Phenomenology of baryon dynamics with directed flow in relativistic heavy-ion collisions"}} submitted by \textbf{Mr. Tribhuban Parida} to the Indian Institute of Science Education and Research (IISER) Berhampur, India for the award of the degree of Doctor of Philosophy has been accepted by the external examiners and that the student has successfully defended the thesis in the viva-voce examination held today.

\vspace{3cm}

\begin{flushright}
    \textbf{Dr. Sandeep Chatterjee} \hfill \textbf{Dr. Sayantan Sharma}  \\
    \textbf{(Thesis Supervisor)}  \hfill  \textbf{(RPC Member)} \\
    \vspace{40mm}
    \textbf{Dr. Md. Nasim} \hfill \textbf{Dr. Ujjal Kumar Dey}  \\
    \textbf{(RPC Member)}  \hfill  \textbf{(RPC Member)} \\
    \vspace{40mm}
    \textbf{External Examiner} \hfill \textbf{ }  \\
    \textbf{  }  \hfill  \textbf{ } \\
   
\end{flushright}



\newpage






\chapter*{CERTIFICATE}

The research work embodied in this thesis entitled \textbf{\textit{"Phenomenology of baryon dynamics with directed flow in relativistic heavy-ion collisions"}} has been carried out under my supervision and is bonafide work of \textbf{Mr. Tribhuban Parida}. This work is original and has not been submitted for any other degree or diploma of this or any other University.


\vspace{5cm}

\begin{flushright}
    \textbf{Date:} \hfill \textbf{Dr. Sandeep Chatterjee}  \\
    \textbf{Odisha, India}  \hfill  \textbf{(PhD Supervisor)} \\
  
\end{flushright}



\newpage



\chapter*{Declaration}
I hereby declare that the research work embodied in this thesis entitled \textbf{\textit{"Phenomenology of baryon dynamics with directed flow in relativistic heavy-ion collisions"}} has been carried out by me at Indian Institute of Science Education and Research (IISER) Berhampur, India under the guidance of \textbf{Dr. Sandeep Chatterjee}, Assistant Professor, Indian Institute of Science Education and Research (IISER) Berhampur, India. I also affirm that this work is original and has not been submitted in part or full for any other degree or diploma to this or any other University or Institution.


\vspace{5cm}

\begin{flushright}
    \textbf{Date:} \hfill \textbf{Tribhuban Parida}  \\
    \textbf{Odisha, India}  \hfill  \textbf{(Candidate)} \\
  
\end{flushright}











%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> institute_format/certificate.tex <==

\chapter*{CERTIFICATE}

The undersigned have examined the Ph.D. thesis entitled:
\vspace{1mm}
\\
\textbf{Phenomenology of baryon dynamics with directed flow in relativistic heavy-ion collisions}
presented by \textbf{Tribhuban Parida}, a candidate for the degree of Doctor of Philosophy in \textbf{Department of Physical Sciences}, and hereby certify that it is worthy of acceptance.


\vspace{2cm} % Adjust space before signatures


\noindent
\textbf{Thesis Supervisor:} \underline{Dr. Sandeep Chatterjee} \hfill \textbf{Signature:} \underline{\hspace{3cm}}

\vspace{1.0cm}


\noindent
\textbf{Thesis Examiner:} \underline{Prof. Subrata Pal} \hfill \textbf{Signature:} \underline{\hspace{3cm}}

\vspace{1.0cm}

\noindent
\textbf{Chairperson:} \underline{Dr. Malay Kumar Rana} \hfill \textbf{Signature:} \underline{\hspace{3cm}}

\vspace{1.0cm}


\clearpage


==> institute_format/declaration.tex <==
\chapter*{ACADEMIC INTEGRITY AND COPYRIGHT DISCLAIMER}
%\begin{SingleSpace}
\begin{quote}
%\utsinitial{I},  
I hereby declare that this thesis is my own work and, to the best of my
knowledge, it contains no materials previously published or written by any
other person, or substantial proportions of material which have been accepted
for the award of any other degree or diploma at IISER Berhampur or any
other educational institution, except where due acknowledgment is made in
the thesis.

I certify that all copyrighted material incorporated into this thesis is in
compliance with the Indian Copyright (Amendment) Act, 2012 and that I have
received written permission from the copyright owners for my use of their
work, which is beyond the scope of the law. I agree to indemnify and save
harmless IISER Berhampur from any and all claims that may be asserted or
that may arise from any copyright violation.
%
%This research is supported by the Australian Government Research Training Program.
% comment from here  xxxxxxxxxxxxxxxx

\noindent

\vspace{1.5cm}
\noindent


\begin{tikzpicture}[remember picture]
\node[anchor=south west] at (0,0) {
%\hspace{1.5cm}\includegraphics[width=0.5\textwidth]{figures/tribubansign.jpg}};
\hspace{1.5cm}\includegraphics[width=0.5\textwidth]{}};


\node[anchor=south west] at (0,0) {
\noindent
\hspace{0.00cm}\textsc{Signature: } \underline{~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~}
};
\node[anchor=south west] at (0,-0.0) {
\noindent

};
\end{tikzpicture}



%\vspace{0.15cm}
%\noindent 
%\hspace{-0.75cm}\textsc{Date: } \DTMsetstyle{en-GB}\DTMdate{\utsyear-\utsmonth-\utsday}
\noindent 
\hspace{0.00cm}\textsc{Date: }  \\
\noindent 
\hspace{0.00cm}\textsc{Place: } {}




\end{quote}
%\end{SingleSpace}
\clearpage


==> institute_format/submission.tex <==
%=========================
% Submission page
%=========================
\begin{titlingpage}
\begin{SingleSpace}

\calccentering{\unitlength} 
\begin{adjustwidth*}{\unitlength}{-\unitlength}
%\vspace*{5mm}
\begin{center}

~\\
\vspace{17mm}

\rule[0.5ex]{\linewidth}{2pt}\vspace*{-\baselineskip}\vspace*{3.2pt}
\rule[0.5ex]{\linewidth}{1pt}\\%[\baselineskip]
\noindent
{\LARGE{A Study on} \\[.25cm] \HUGE{\utstitle}} \\[1.5mm] % Title
%{\Large \textit{Subtitle}}\\
\rule[0.5ex]{\linewidth}{1pt}\vspace*{-\baselineskip}\vspace{4pt}
\rule[0.5ex]{\linewidth}{2pt}\\
\vspace {15mm}
%{\large By}\\
%\vspace{6.5mm}

\emph{\large A thesis submitted in partial fulfilment of the requirements}\\
\vspace {0.1in}
\emph{\large for the award of the degree of}\\
\vspace {10mm}
{\large \textbf{Doctor of Philosophy}}\\
\vspace{2mm}
%\emph{in}\\
%\vspace{1mm}
%{\large \utsfield}\\
\vspace {8mm}
\emph{\large by}\\
\vspace{4mm}
{\bfseries \Large \utsname} \\ % Author
\vspace{2mm}
{\textbf{Registration Number- 1920503}}

\vspace {10mm}
\emph{\large to the }\\
\vspace{4mm}
{
\vspace {1mm}
\vspace {2mm}
{\Large Department of Physical Sciences}\\
\vspace{2mm}
{\Large Indian Institute of Science Education and Research (IISER) Berhampur}\\
\vspace {1mm}
{India}
}\\
\begin{figure}[h]
    \centering
    \includegraphics[width=0.3\textwidth]{assets/Logo_iiserbpr.png}
\end{figure}

\vspace{10mm}

{\large{\DTMenglishmonthname{\utsmonth}~\utsyear}}
\end{center}
\end{adjustwidth*}

% end submission page
%================================================================
\clearpage

%=========================
% Copyright
%=========================
\pagestyle{empty}
\null\vfill
%\vskip 60\p@
\begin{center}
  {\textcopyright}~{\utsyear} by \href{utsurl}{\utsname}
  \\All Rights Reserved
\end{center}
\end{SingleSpace}
\end{titlingpage}

==> institute_format/title.tex <==
%=======================================
{
\pagestyle{empty}
\changepage{5cm}{1cm}{-0.5cm}{-0.5cm}{}{-2cm}{}{}{}
\vspace{7mm}

%=======================================
% Title page
%=======================================

% Header
%{\small
%\noindent 
%\textit{\utscoursecode: Doctor of Philosophy}\\
%\textit{PhD Thesis: \utsfield}\\
%\noindent 
%\textit{\DTMenglishmonthname{\utsmonth}~\utsyear}
%}



\par\vspace{6.5cm}
% end header

% Title
\begin{center}
  {\LARGE\emph{A Study on}}\\
  \vskip 0.5cm
  {\Huge\bfseries \utstitle}
  \\[0.4cm]
  \rule{\textwidth}{1.5pt}  % Thicker rule with better spacing
\end{center}
% end title
%=================

\begin{center}
  {\LARGE \textbf{\utsname}}\\
  \vskip 1cm
  \textit{A thesis submitted in partial fulfillment of}\\
  \textit{the requirements for the degree of}\\
  \vskip 0.3cm
  \textbf{Doctor of Philosophy}\\
  %\textbf{\DTMenglishmonthname{\utsmonth}~\utsyear}
\end{center}

\vfill

\begin{center}
  \includegraphics[height=2cm]{assets/Logo_IISER.png}  % Add logo if available
  \vskip 0.5cm
  \textbf{\Large Indian Institute of Science Education and Research (IISER) Berhampur}\\
  \vskip 0.2cm
  \textit{India}
\end{center}

% Footer
\vfill  % Flexible vertical space

% Department/Faculty information
\begin{center}
  \textit{Supervisor: Dr. Md. Nasim}  % Add supervisor if required
  \\[0.5cm]
  \textsc{Department of \utsfield}\\
  Indian Institute of Science Education and Research (IISER) Berhampur
\end{center}


\noindent%
%{
%Indian Institute of Science Education and Research (IISER) Berhampur, 
%India}
% end footer
\clearpage
}

\utsclearemptydoublepage % this is here on purpose!

